CP violation observables in baryon decays

The era of baryon physics is on the horizon with the accumulation of increasing data by collaborations such as LHCb, Belle II, and BESIII. Despite the wealth of data, one of the critical issues in flavor physics, namely CP violation in baryon decays, still awaits experimental confirmation. It is evident that the development of formulas and phenomenological analyses will play a pivotal role in advancing theoretical investigations and experimental measurements in this domain. In this work, we discuss the fundamental definitions and properties of polarization, asymmetry parameters and their associated CP violating observables that may arise in baryon decays. Additionally, we provide a detailed analysis of b-baryon quasi-two and -three body decays based on angular distributions. We highlight the significance of CP asymmetries defined by spin and momentum correlations, as non-trivial spin distributions are expected in baryon decays due to their non-zero polarization in productions and decays. Of particular importance is a complementary relation can be establised for two different types of observables, that are $\mathcal{T}$-even and -odd CP asymmetries respectively. The complementarity indicates that one observable exhibits the sine dependence on strong phase $\Delta\delta$, while another exhibits as cosine. This gives us an distinctive opportunity to avoid the potential large suppression to CP asymmetries from small phase $\Delta\delta$. Two points (\textbf{i}) the exact proof of strong phase dependence behaviour, and (\textbf{ii}) the criterion for complementary observables are clarified. Based on these arguments from theoretical aside, some brief discussions and suggestions on experimental measurements are offered in the final discussions. Lastly, we present a pedagogical introduction to angular distribution techniques based on helicity descriptions for both two and three body decays.

==> abundant.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$\Lambda_b^{0*}\to \Lambda_b^0\pi^+\pi^-$}
\begin{itemize}
\item {Please add the discussions on $\Lambda_b^*\to \Lambda_b^0\pi^+\pi^-$. Give any CPV observables, no matter whether it is proportional to $\sin\delta$ or $\cos\delta$. Any of them is a new observable. }
\item { Standing in the viewpoint of kinematics, the cascade decay $\Lambda_b^{0*}\to \Lambda_b^0\pi^+\pi^-$ with $\Lambda_{b}\to p\pi/K$ is comparable with quasi-two-body decays. Therefore, we can investigate it from corresponding differentiate distribution. In the frame of excited baryon $\Lambda_{b}^{*}$, the distribution of this decay is expressed as helicity amplitudes and Wigner D function
\begin{equation}
		\begin{aligned}
        \mathcal{W}(\theta,\phi)\propto \sum_{\lambda,\lambda^{\prime},m}\mathcal{H}_{S}(\lambda)\mathcal{H}^{*}_{S}(\lambda^{\prime})D^{j=+\frac{1}{2}}_{\lambda,m}(\theta,\phi)D^{*j=+\frac{1}{2}}_{\lambda^{\prime},m}(\theta,\phi)\left|h_{m}\right|^{2}\delta_{\lambda,\lambda^{\prime}}
		\end{aligned}
\end{equation}
where $\mathcal{H}_{S}(\lambda)$ is helicity amplitude of strong decay $\Lambda_b^{0*}\to \Lambda_b^0\pi^+\pi^-$ and $h_{m}$ denotes the magnitude of weak decay $\Lambda_{b}\to p\pi/K$. Explicitly, we find
\begin{equation}\label{eq:Lbstar}
\begin{aligned}
\mathcal{W}(\theta,\phi)\propto\left|\mathcal{H}_{S}\right|^{2}\times \left|\mathcal{H}_{W}\right|^{2}
\end{aligned}
\end{equation}
when we integrate out redundant angles appearing in $\mathcal{H}_{S}$. Consequently, the strong and weak decay can be completely separated such that there is no observable which we want. One may argue that it is not necessary to appoint the helicity of $\Lambda_{b}^{*}$ and $\Lambda_{b}$ in the same direction. However, it would make no sense because it is different from $e^{+}e^{-}$ collision where production process can be determined in the experiment. }

{\color{red}I still can not understand it. What is the main difference between $\Lambda_b^*\to \Lambda_b\pi\pi$ and $\Lambda_b\to pa_1$?  In the latter one, there is a CPV observable related to the angle $\cos\theta$. 
For example, in $\Lambda_b\to p a_1$, the term proportional to $\cos\theta$ is $|\mathcal{H}_{-1,-1/2}|^2-|\mathcal{H}_{+1,+1/2}|^2$. In $B\to K_1\gamma$, the term proportional to $\cos\theta$ is $|A_R|^2-|A_L|^2$. Bot the them are the difference between two helicity amplitudes. The physical meaning is to measure the parity violation, which can also be seen by  $\cos\theta$. They are exactly the same as $\alpha$.

Now back to $\Lambda_b^*\to \Lambda\pi\pi$, do you think it is possible to measure a parity-odd observable proportional to $|\mathcal{H}_{-1/2,-1/2}|^2-|\mathcal{H}_{+1/2,+1/2}|^2$ with the helicity amplitudes corresponding to $\Lambda_b\to p\pi$ decays. Please look at Eq.(\ref{eq:Lbstar}) more carefully, and see whether it is something like $|\mathcal{H}_S|^2\times(|\mathcal{H}_{-1/2,-1/2}|^2-|\mathcal{H}_{+1/2,+1/2}|^2)$? 

The angular distributions must be related to the proton momentum in the $\Lambda_b^*$ rest frame. The quantity of $\vec n\cdot \vec p_p$, with $\vec n$ as the normal vector of the $\Lambda_b^*\to \Lambda_b\pi\pi$ plane and $\vec p_p$ as the proton momentum in the $\Lambda_b^*$ rest frame, is a parity odd quantity. 

The problem is that the proton momentum is always used in the $\Lambda_b$ rest frame, but now it should be in the $\Lambda_b^*$ frame. We should boost the proton momentum. Otherwise, can we construct a similar CP-odd quantity in the $\Lambda_b$ rest frame?
}

\item The signal events of $\Lambda_b^{**}(6070)\to\Lambda_b\pi\pi$ with $\Lambda_b^0\to p J/\Psi K^-$ are $550\pm80$ using the LHCb data of 9 fb$^{-1}$ \cite{LHCb:2020lzx}. Considering the branching fractions of $Br(\Lambda_b\to p J/\Psi K^-)Br(J/\Psi\to \mu^+\mu^-)=(3.2^{+0.6}_{-0.5})\times10^{-4}\times6\%\sim2\times10^{-5}$ and $Br(\Lambda_b\to pK^-)=(5.4\pm1.0)\times10^{-6}$, the signal events of $\Lambda_b^{**}(6070)\to\Lambda_b\pi\pi$ with $\Lambda_b^0\to p K^-$ would be at the order of one hundred. Combining more resonances, the signal events could be even larger, such as $N(\Lambda_b^{*}(5912)\to\Lambda_b\pi\pi)=57\pm9$, $N(\Lambda_b^{*}(5920)\to\Lambda_b\pi\pi)=204\pm17$, $N(\Lambda_b^{*}(6146)\to\Lambda_b\pi\pi)=103\pm22$ and $N(\Lambda_b^{*}(6152)\to\Lambda_b\pi\pi)=90\pm21
$, with $\Lambda_b^0\to p J/\Psi K^-$ \cite{LHCb:2020lzx}.

\item {\color{red} Another question related  not only to $\Lambda_b^*\to \Lambda_b\pi\pi$ but also to $\Lambda_b\to pa_1$, the parity-odd quantity is $\vec n\cdot \vec p$, which is very similar to $\alpha$ for $\vec \sigma\codt\vec p$. Do you think we can measure a quantity of $\vec n\times \vec p$, just like $\beta$ for $\vec \sigma\times \vec p$?
}
\item{\color{blue} Yes, there is observable like $\vec n\times \vec p$. The observable $sin\varphi$ in the decay $\Lambda_{b}\to N^{*}(3/2)\rho$ has been proved as the form of $\vec n\times \vec p$. When we consider the decay $\Lambda_{b}^{*}\to \Lambda_{b}\pi\pi$, there is no CP violation observable like this.} {\color{red}(FSY: No, $\sin\varphi$ is something like $\vec n\cdot \vec p$, but not $\vec n\times \vec p$. See Eq.(\ref{eq:sinphi-TPA}).)}
\end{itemize}



\item{\color{red}It seems that we can measure the transverse polarization of proton, i.e. $\beta$, in $\Lb\to p\pim$ using the transverse polarization of $\Lb$. Or similarly for $\Lz\to p\pim$. We take $\Lz\to p\pim$ as an example. Now we have three independent directions, the momentum of $\Lz$, the momentum of proton, and the transverse polarization of $\Lz$. In the measurement of $\alpha$, we actually only have two directions, the longitudinal polarization of $\Lz$ and the momentum of proton. The momentum of $\Lz$ is in the same direction of its longitudinal polarization. In this case, we can only construct one observable, $\vec\sigma_L\cdot \vec p_p$. Here we take $\vec\sigma_{T,L}$ as the transverse and longitudinal polarizations.  The transverse polarization of proton might by measured by $(\vec\sigma_T\times\vec p_p)\cdot(\vec p_\Lambda\times\vec p_p)$, which is a $P$-odd observable. Both of $(\vec\sigma_T\times\vec p_p)$ and $(\vec p_\Lambda\times\vec p_p)$ are in the transverse plane of proton. 

So do you think this observable can be used to measure $\beta$? If so, we can use it to measure the $\beta$ of $\Lb\to p\pi$ and $pK$. The problem might be how to express this observable by the helicity amplitudes? Or whether is it the $\beta$ what we want? Since the directions in $(\vec\sigma_T\times\vec p_p)\cdot(\vec p_\Lambda\times\vec p_p)$ might be different from the definition of $\beta$, it is possible a combination of $\beta$ and $\gamma$. So could we find an observable which is exactly the $\beta$?}

